Tubings, chord diagrams, and Dyson--Schwinger equations

We give series solutions to single insertion place propagator-type systems of Dyson--Schwinger equations using binary tubings of rooted trees. These solutions are combinatorially transparent in the sense that each tubing has a straightforward contribution. The Dyson--Schwinger equations solved here are more general than those previously solved by chord diagram techniques, including systems and non-integer values of the insertion parameter $s$. We remark on interesting combinatorial connections and properties.

==> figure_cdip_insertion2.tex <==
% (CC BY-SA 4.0 https://creativecommons.org/licenses/by-sa/4.0/) Paul Balduf, November 2022. Please cite the original paper as a source when reusing this drawing.


\begin{tikzpicture}[hl/.style={violet}]

        \node at (-1,.3) {$C'=$};
        \coordinate (c1) at ($  (0,0)$){};
        \coordinate (c2) at ($(c1) + (.8,0)$){};
        \coordinate (c3) at ($(c2) + (.8,0)$){};
        \coordinate (c4) at ($(c3) + (.8,0)$){};
        \coordinate (c5) at ($(c4) + (.8,0)$){};
        \coordinate (c6) at ($(c5) + (.8,0)$){};

		\node at ($(c1)!.5!(c2) + (270:.1)$) {\color{blue}\scriptsize $y_1$};
		\node at ($(c2)!.5!(c3) + (270:.1)$) {\color{blue}\scriptsize $y_2$};
		\node at ($(c3)!.5!(c4) + (270:.1)$) {\color{blue}\scriptsize $y_3$};
		\node at ($(c4)!.5!(c5) + (270:.1)$) {\color{blue}\scriptsize $y_4$};
		\node at ($(c5)!.5!(c6) + (270:.1)$) {\color{blue}\scriptsize $y_5$};

		\draw[chord, blue] (c1) to (c3);
		\draw[chord, blue] (c2) to (c5);
		\draw[chord, blue] (c4) to (c6);
		
		 \node at (6.5,.3) {$C''=$};
		\coordinate (c1) at ($  (7.5,0)$){};
		\coordinate (c2) at ($(c1) + (.8,0)$){};
		\coordinate (c3) at ($(c2) + (.8,0)$){};
		\coordinate (c4) at ($(c3) + (.8,0)$){};
		\coordinate (c5) at ($(c4) + (.8,0)$){};
		\coordinate (c6) at ($(c5) + (.8,0)$){};
		
		\node at ($(c1)!.5!(c2) + (270:.1)$) {\scriptsize $y_1$};
		\node at ($(c2)!.5!(c3) + (270:.1)$) {\scriptsize $y_2$};
		\node at ($(c3)!.5!(c4) + (270:.1)$) {\scriptsize $y_3$};
		\node at ($(c4)!.5!(c5) + (270:.1)$) {\scriptsize $y_4$};
		\node at ($(c5)!.5!(c6) + (270:.1)$) {\scriptsize $y_5$};
		
		\draw[chord, black] (c1) to (c4);
		\draw[chord, black] (c2) to (c6);
		\draw[chord, black] (c3) to (c5);
		
		\node at (0,-2.7) {$C=$};
		\coordinate (c1) at ($  (1,-3)$){};
		\coordinate (c2) at ($(c1) + (.8,0)$){};
		\coordinate (c3) at ($(c2) + (.8,0)$){};
		\coordinate (c4) at ($(c3) + (.8,0)$){};
		\coordinate (c5) at ($(c4) + (.8,0)$){};
		\coordinate (c6) at ($(c5) + (.8,0)$){};
		\coordinate (c7) at ($(c6) + (.8,0)$){};
		\coordinate (c8) at ($(c7) + (.8,0)$){};
		\coordinate (c9) at ($(c8) + (.8,0)$){};
		\coordinate (c10) at ($(c9) + (.8,0)$){};
		\coordinate (c11) at ($(c10) + (.8,0)$){};
		\coordinate (c12) at ($(c11) + (.8,0)$){};
		
		\node at ($(c1)!.5!(c2) + (270:.1)$) {\scriptsize $y_1$};
		\node at ($(c2)!.5!(c3) + (270:.1)$) {\scriptsize $y_2$};
		\node at ($(c3)!.5!(c4) + (270:.1)$) {\scriptsize $y_3$};
		\node at ($(c4)!.5!(c5) + (270:.1)$) {\scriptsize $y_4$};
		\node at ($(c5)!.5!(c6) + (270:.1)$) {\scriptsize $y_5$};
		\node at ($(c6)!.5!(c7) + (270:.1)$) {\color{blue}\scriptsize $y_6$};
		\node at ($(c7)!.5!(c8) + (270:.1)$) {\color{blue}\scriptsize $y_7$};
		\node at ($(c8)!.5!(c9) + (270:.1)$) {\color{blue}\scriptsize $y_8$};
		\node at ($(c9)!.5!(c10) + (270:.1)$) {\color{blue}\scriptsize $y_9$};
		\node at ($(c10)!.5!(c11) + (270:.1)$) {\scriptsize $y_{10}$};
		\node at ($(c11)!.5!(c12) + (270:.1)$) {\scriptsize $y_{11}$};
		
		\draw[chord, blue] (c1) to (c7);
		\draw[chord, blue] (c6) to (c9);
		\draw[chord, blue] (c8) to (c10);
		\draw[chord, black] (c2) to (c5);
		\draw[chord, black] (c3) to (c12);
		\draw[chord, black] (c4) to (c11);


\end{tikzpicture}
